Composite Re-Ranking for Efficient Document Search with BERT

Although considerable efforts have been devoted to transformer-based ranking models for document search, the relevance-efficiency tradeoff remains a critical problem for ad-hoc ranking. To overcome this challenge, this paper presents BECR (BERT-based Composite Re-Ranking), a composite re-ranking scheme that combines deep contextual token interactions and traditional lexical term-matching features. In particular, BECR exploits a token encoding mechanism to decompose the query representations into pre-computable uni-grams and skip-n-grams. By applying token encoding on top of a dual-encoder architecture, BECR separates the attentions between a query and a document while capturing the contextual semantics of a query. In contrast to previous approaches, this framework does not perform expensive BERT computations during online inference. Thus, it is significantly faster, yet still able to achieve high competitiveness in ad-hoc ranking relevance. Finally, an in-depth comparison between BECR and other start-of-the-art neural ranking baselines is described using the TREC datasets, thereby further demonstrating the enhanced relevance and efficiency of BECR.

==> tables.tex <==
\begin{table*}[htbp!]
	\caption{Relevance comparison of Bexr against baselines}
	\centering
	\begin{small}
		%\resizebox{2.0\columnwidth}{!}{
		\begin{tabular}{c || c | c | c | c || c | c | c | c}
			\toprule
			Model 	& \multicolumn{4}{|c||}{ClueWeb09-Cat-B} 		& \multicolumn{4}{|c}{Robust04} 			\\
							   		  		NDCG@k	& 1 & 3 & 5 & 10 	& 1 & 3 & 5 & 10 	\\
 			\midrule
			BM25	&  0.2437 & 0.2357 & 0.2351 & 0.2320 & 0.5505 & 0.5505 & 0.4594 & 0.4370\\
			CONV-KNRM 	& 0.2842 & 0.2857 & 0.2869 & 0.2859 & 0.5373 & 0.4875 & 0.4875 & 0.4875\\
			BERT & 0.3190 & 0.2897 & 0.2853 & 0.2773 & 0.5721 & 0.5423 & 0.5160 & 0.4774\\
			CEDR-KNRM & 0.3137 & 0.3037 & 0.3030 & 0.2909 & 0.6206 & 0.5847 & 0.5563 & 0.5078\\
			\midrule
			Bexr-partial &  0.3139 & 0.3064 & 0.3110 & 0.2930 & 0.6089& 0.5631& 0.5366& 0.4955\\
			Bexr-full &   0.2914 & 0.2885 & 0.2965 & 0.2793 &  0.5626 & 0.5078 & 0.4914 & 0.4562 \\
			\bottomrule
		\end{tabular}
		%}
		\label{tab:main}
	\end{small}
\end{table*}

